Data Augmentation by AutoEncoders for Unsupervised Anomaly Detection

This paper proposes an autoencoder (AE) that is used for improving the performance of once-class classifiers for the purpose of detecting anomalies. Traditional one-class classifiers (OCCs) perform poorly under certain conditions such as high-dimensionality and sparsity. Also, the size of the training set plays an important role on the performance of one-class classifiers. Autoencoders have been widely used for obtaining useful latent variables from high-dimensional datasets. In the proposed approach, the AE is capable of deriving meaningful features from high-dimensional datasets while doing data augmentation at the same time. The augmented data is used for training the OCC algorithms. The experimental results show that the proposed approach enhance the performance of OCC algorithms and also outperforms other well-known approaches.

==> Figures/Plots.tex <==
\begin{figure*}[h!]
\begin{subfigure}{.5\textwidth}
  \centering
  % include first image
  \includegraphics[width=.8\linewidth]{Figures/plot_ADASYN.png}  
  \caption{Augmented by ADASYN}
  \label{fig:sub-first}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
  \includegraphics[width=.8\linewidth]{Figures/plot_SMOTE.png}  
  \caption{Augmented by SMOTE}
  \label{fig:sub-second}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include 3rd image
  \includegraphics[width=.8\linewidth]{Figures/plot_Noise.png}  
  \caption{Augmented by Noise}
  \label{fig:sub-second}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include 3rd image
  \includegraphics[width=.8\linewidth]{Figures/plot_Proposed_approach.png}  
  \caption{Augmented by Proposed Model}
  \label{fig:sub-second}
\end{subfigure}
\caption{Plotting the first two features ($Z_0$ and $Z_1$) of the hidden variables obtained from the PenDigits data set after data augmentation}
\label{fig:plots}
\end{figure*}

==> Tables/ADASYN.tex <==
\begin{table*}[h]
\caption{AUC and APR from AE-ADASYN-OCC}
\label{tab:auc_AE-ADASYN-OCC}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|l|l|l|l|l|l|l|}
\multirow{2}{*}{Dataset name} & \multirow{2}{*}{Attack} & \multicolumn{2}{c|}{Isolation Forest} & \multicolumn{2}{c|}{KDE} & \multicolumn{2}{c|}{LOF} \\ \cline{3-8} 
 &  & \multicolumn{1}{c|}{PR AUC} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{PR AUC} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{PR AUC} & \multicolumn{1}{c|}{AUC} \\ \hline
UNSW & Fuzzers & 0.848214 & 0.489391 & 0.882237 & 0.522690 & 0.837457 & 0.440378 \\
UNSW & Analysis & 0.992451 & 0.810318 & 0.985799 & 0.687999 & 0.969598 & 0.376012 \\
UNSW & Backdoor & 0.995076 & 0.784588 & 0.995298 & 0.834569 & 0.987576 & 0.585176 \\
UNSW & DoS & 0.964019 & 0.748114 & 0.960431 & 0.703658 & 0.834013 & 0.352290 \\
UNSW & Exploits & 0.718556 & 0.427573 & 0.743269 & 0.496424 & 0.734920 & 0.385098 \\
UNSW & Generic & 0.921261 & 0.822522 & 0.902204 & 0.777814 & 0.662461 & 0.523091 \\
UNSW & Reconnaissance & 0.894527 & 0.525260 & 0.934191 & 0.560724 & 0.891446 & 0.346297 \\
UNSW & Shellcode & 0.985252 & 0.470260 & 0.993044 & 0.554383 & 0.986891 & 0.341107 \\
UNSW & Worms & 0.999022 & 0.475963 & 0.999468 & 0.671306 & 0.998885 & 0.527491 \\
Spambase & NaN & 0.313269 & 0.376849 & 0.348382 & 0.400800 & 0.331663 & 0.386958 \\
Shuttle & NaN & 0.727886 & 0.400832 & 0.690291 & 0.356852 & 0.763299 & 0.597993 \\
NSLKDD & Probe & 0.831492 & 0.574968 & 0.953483 & 0.862591 & 0.625817 & 0.097050 \\
NSLKDD & DoS & 0.872377 & 0.924227 & 0.856578 & 0.910664 & 0.369592 & 0.070943 \\
NSLKDD & R2L & 0.906949 & 0.736042 & 0.938737 & 0.775114 & 0.636912 & 0.222205 \\
NSLKDD & U2R & 0.998072 & 0.762937 & 0.997940 & 0.808469 & 0.977794 & 0.047458 \\
InternetAds & NaN & 0.168142 & 0.525253 & 0.148903 & 0.443780 & 0.127709 & 0.374203 \\
CTU13-13 & Virut & 0.374854 & 0.067134 & 0.364312 & 0.089389 & 0.455612 & 0.312764 \\
CTU13-10 & Rbot & 0.729685 & 0.017754 & 0.696497 & 0.004629 & 0.696123 & 0.004044 \\
CTU13-09 & Neris & 0.729915 & 0.117373 & 0.751907 & 0.286454 & 0.750559 & 0.222370 \\
CTU13-08 & Murlo & 0.063167 & 0.037699 & 0.042349 & 0.047424 & 0.044261 & 0.166757 \\
PenDigits & NaN & 0.725999 & 0.715656 & 0.454848 & 0.452025 & 0.388993 & 0.215232 \\
Arrhythmia & NaN & 0.373102 & 0.365440 & 0.377171 & 0.392179 & 0.376357 & 0.382979     
\end{tabular}%
}
\end{table*}


==> Tables/AE-OCC_no_oversampling.tex <==
\begin{table*}[h]
\caption{AUC and APR from AE-OCC without over-sampling}
\label{tab:auc_ae-occ_no_os}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|l|l|l|l|l|l|l|}
\multirow{2}{*}{Dataset name} & \multirow{2}{*}{Attack} & \multicolumn{2}{c|}{Isolation Forest} & \multicolumn{2}{c|}{KDE} & \multicolumn{2}{c|}{LOF} \\ \cline{3-8} 
 &  & \multicolumn{1}{c|}{PR AUC} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{PR AUC} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{PR AUC} & \multicolumn{1}{c|}{AUC} \\ \hline
UNSW & Fuzzers & 0.825036 & 0.478908 & 0.821277 & 0.456699 & 0.837677 & 0.437893 \\
UNSW & Analysis & 0.995042 & 0.782159 & 0.993381 & 0.800109 & 0.996523 & 0.847938 \\
UNSW & Backdoor & 0.996072 & 0.813686 & 0.995197 & 0.787838 & 0.985830 & 0.475697 \\
UNSW & DoS & 0.949991 & 0.689533 & 0.956078 & 0.682029 & 0.843360 & 0.402249 \\
UNSW & Exploits & 0.758706 & 0.502675 & 0.744395 & 0.412457 & 0.693678 & 0.515871 \\
UNSW & Generic & 0.939197 & 0.878795 & 0.810372 & 0.671945 & 0.693678 & 0.515871 \\
UNSW & Reconnaissance & 0.914804 & 0.531217 & 0.921504 & 0.552506 & 0.877878 & 0.349491 \\
UNSW & Shellcode & 0.990140 & 0.476668 & 0.992143 & 0.519254 & 0.985469 & 0.332977 \\
UNSW & Worms & 0.999221 & 0.603508 & 0.998785 & 0.421189 & 0.998178 & 0.328157 \\
Spambase & NaN & 0.341589 & 0.418196 & 0.360805 & 0.459930 & 0.332024 & 0.396404 \\
Shuttle & NaN & 0.826543 & 0.686794 & 0.697959 & 0.406156 & 0.791192 & 0.473181 \\
NSLKDD & Probe & 0.973640 & 0.911605 & 0.980573 & 0.917920 & 0.648103 & 0.168020 \\
NSLKDD & DoS & 0.864187 & 0.827056 & 0.878124 & 0.885334 & 0.506144 & 0.388560 \\
NSLKDD & R2L & 0.926457 & 0.761338 & 0.834977 & 0.723810 & 0.656435 & 0.230689 \\
NSLKDD & U2R & 0.999189 & 0.889441 & 0.999283 & 0.905428 & 0.979952 & 0.075275 \\
InternetAds & NaN & 0.116430 & 0.317850 & 0.163271 & 0.532562 & 0.125463 & 0.376130 \\
CTU13-13 & Virut & 0.371459 & 0.057874 & 0.516925 & 0.269013 & 0.917601 & 0.945368 \\
CTU13-10 & Rbot & 0.749819 & 0.033867 & 0.703082 & 0.041395 & 0.696685 & 0.008857 \\
CTU13-09 & Neris & 0.709616 & 0.078740 & 0.762619 & 0.286242 & 0.757087 & 0.244064 \\
CTU13-08 & Murlo & 0.045257 & 0.051229 & 0.041883 & 0.091475 & 0.121086 & 0.724943 \\
PenDigits & NaN & 0.951352 & 0.944919 & 0.962761 & 0.932840 & 0.603401 & 0.398374 \\
Arrhythmia & NaN & 0.396966 & 0.364290 & 0.461485 & 0.336975 & 0.398164 & 0.359689
\end{tabular}%
}
\end{table*}



==> Tables/Oversampling_by_AE.tex <==
\begin{table*}[h]
\caption{AUC and APR from the proposed method}
\label{tab:Oversampling_with_AE}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|l|l|l|l|l|l|l|}
\multirow{2}{*}{Dataset name} & \multirow{2}{*}{Attack} & \multicolumn{2}{c|}{Isolation Forest} & \multicolumn{2}{c|}{KDE} & \multicolumn{2}{c|}{LOF} \\ \cline{3-8} 
 &  & \multicolumn{1}{c|}{PR AUC} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{PR AUC} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{PR AUC} & \multicolumn{1}{c|}{AUC} \\ \hline
UNSW & Fuzzers & 0.892541 & 0.566919 & 0.932162 & 0.668255 & 0.875147 & 0.540312 \\
UNSW & Analysis & 0.996924 & 0.851430 & 0.995841 & 0.814133 & 0.992412 & 0.801947 \\
UNSW & Backdoor & 0.998410 & 0.924112 & 0.998104 & 0.905562 & 0.995823 & 0.842277 \\
UNSW & DoS\_UNSW & 0.970271 & 0.826416 & 0.974393 & 0.821914 & 0.972253 & 0.830417 \\
UNSW & Exploits & 0.873707 & 0.681366 & 0.868570 & 0.649352 & 0.792443 & 0.642762 \\
UNSW & Generic & 0.970416 & 0.943954 & 0.975920 & 0.959502 & 0.861622 & 0.787470 \\
UNSW & Reconnaissance & 0.948154 & 0.591864 & 0.954099 & 0.641890 & 0.954615 & 0.718356 \\
UNSW & Shellcode & 0.995799 & 0.680610 & 0.988500 & 0.467794 & 0.990512 & 0.496891 \\
UNSW & Worms & 0.999559 & 0.713073 & 0.999377 & 0.605728 & 0.995850 & 0.133606 \\
Spambase & NaN & 0.675825 & 0.774560 & 0.650758 & 0.809145 & 0.658838 & 0.768035 \\
Shuttle & NaN & 0.875430 & 0.721399 & 0.807903 & 0.643564 & 0.969470 & 0.896950 \\
NSLKDD & Probe & 0.986279 & 0.941792 & 0.991266 & 0.972700 & 0.745125 & 0.494517 \\
NSLKDD & DoS & 0.930527 & 0.917002 & 0.954689 & 0.931012 & 0.570047 & 0.590169 \\
NSLKDD & R2L & 0.977382 & 0.918996 & 0.969043 & 0.887017 & 0.798307 & 0.593956 \\
NSLKDD & U2R & 0.999088 & 0.881643 & 0.998885 & 0.862695 & 0.987738 & 0.423325 \\
InternetAds & NaN & 0.169031 & 0.466906 & 0.201999 & 0.561736 & 0.165670 & 0.467504 \\
CTU13-13 & Virut & 0.619064 & 0.535564 & 0.491265 & 0.391861 & 0.906059 & 0.873392 \\
CTU13-10 & Rbot & 0.946248 & 0.668767 & 0.834443 & 0.617867 & 0.993069 & 0.961478 \\
CTU13-09 & Neris & 0.834648 & 0.455843 & 0.928739 & 0.600368 & 0.928190 & 0.682503 \\
CTU13-08 & Murlo & 0.087592 & 0.185086 & 0.063823 & 0.103915 & 0.048526 & 0.217836 \\
PenDigits & NaN & 0.983164 & 0.976978 & 0.962094 & 0.932552 & 0.989877 & 0.988474 \\
Arrhythmia & NaN & 0.482648 & 0.444221 & 0.500965 & 0.554054 & 0.500965 & 0.554054  
\end{tabular}%
}
\end{table*}


==> Tables/SMOTE.tex <==
\begin{table*}[h]
\caption{AUC and APR from AE-SMOTE-OCC}
\label{tab:auc_AE-SMOTE-OCC}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|l|l|l|l|l|l|l|}
\multirow{2}{*}{Dataset name} & \multirow{2}{*}{Attack} & \multicolumn{2}{c|}{Isolation Forest} & \multicolumn{2}{c|}{KDE} & \multicolumn{2}{c|}{LOF} \\ \cline{3-8} 
 &  & \multicolumn{1}{c|}{PR AUC} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{PR AUC} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{PR AUC} & \multicolumn{1}{c|}{AUC} \\ \hline
UNSW & Fuzzers & 0.811112 & 0.390783 & 0.794023 & 0.393841 & 0.792758 & 0.285240 \\
UNSW & Analysis & 0.992678 & 0.718894 & 0.989924 & 0.685089 & 0.962176 & 0.240545 \\
UNSW & Backdoor & 0.995121 & 0.844325 & 0.993861 & 0.726301 & 0.971901 & 0.311190 \\
UNSW & DoS & 0.942951 & 0.664335 & 0.945166 & 0.718132 & 0.853746 & 0.436574 \\
UNSW & Exploits & 0.838391 & 0.624191 & 0.785510 & 0.527567 & 0.710958 & 0.466195 \\
UNSW & Generic & 0.929252 & 0.834460 & 0.927067 & 0.817085 & 0.718771 & 0.622917 \\
UNSW & Reconnaissance & 0.909179 & 0.467903 & 0.928092 & 0.502661 & 0.841331 & 0.275937 \\
UNSW & Shellcode & 0.984981 & 0.280533 & 0.987357 & 0.349399 & 0.982076 & 0.295315 \\
UNSW & Worms & 0.999615 & 0.748095 & 0.997799 & 0.363395 & 0.996404 & 0.104645 \\
Spambase & NaN & 0.341771 & 0.461088 & 0.318327 & 0.351116 & 0.314642 & 0.332878 \\
Shuttle & NaN & 0.784436 & 0.511532 & 0.628055 & 0.130929 & 0.711398 & 0.364397 \\
NSLKDD & Probe & 0.976404 & 0.900740 & 0.967594 & 0.880886 & 0.627182 & 0.082211 \\
NSLKDD & DoS & 0.728428 & 0.765312 & 0.795510 & 0.863718 & 0.382157 & 0.132857 \\
NSLKDD & R2L & 0.950769 & 0.829185 & 0.938982 & 0.785509 & 0.626956 & 0.187647 \\
NSLKDD & U2R & 0.997571 & 0.715080 & 0.997478 & 0.698844 & 0.980256 & 0.078485 \\
InternetAds & NaN & 0.134174 & 0.411749 & 0.171171 & 0.525253 & 0.165939 & 0.489899 \\
CTU13-13 & Virut & 0.374696 & 0.067515 & 0.370150 & 0.116333 & 0.585436 & 0.651219 \\
CTU13-10 & Rbot & 0.776060 & 0.030359 & 0.698850 & 0.018972 & 0.718925 & 0.065738 \\
CTU13-09 & Neris & 0.738282 & 0.155504 & 0.756732 & 0.260608 & 0.834836 & 0.312507 \\
CTU13-08 & Murlo & 0.061380 & 0.071147 & 0.041370 & 0.086778 & 0.104715 & 0.658943 \\
PenDigits & NaN & 0.557366 & 0.371303 & 0.602315 & 0.587799 & 0.319593 & 0.103495 \\
Arrhythmia & NaN & 0.438593 & 0.443071 & 0.440476 & 0.50000 & 0.419372 & 0.461185
\end{tabular}%
}
\end{table*}
